Optimal transport based theory for latent structured models

This article is an exposition on some recent theoretical advances in learning latent structured models, with a primary focus on the fundamental roles that optimal transport distances play in the statistical theory. We aim at what may be the most critical and novel ingredient in this theory: the motivation, formulation, derivation and ramification of inverse bounds, a rich collection of structural inequalities for latent structured models which connect the space of distributions of unobserved structures of interest to the space of distributions for observed data. This theory is illustrated on classical mixture models, as well as the more modern hierarchical models that have been developed in Bayesian statistics, machine learning and related fields.

==> information_geometry.tex <==
\subsection{Information geometry of finite mixture models}
\label{sec:infgeo}
In this section we present an improvement to the inverse bounds obtained in Theorem \ref{thm:inversebound}, by relating the $\Phi$-distance of mixture densities to the moment difference distance of mixing measures. We establish not only an lower bound, but also an upper bound and therefore characterizes the local geometry of mixture distributions in terms of the moment difference. 

\begin{thm} 
\label{thm:inverseboundmoment}
If $\Theta\subset \Rb^q$ is compact.
\begin{enumerate}[label=(\alph*)]

\item \label{itema:thm:inverseboundmoment}
If $\myF$ is a $(2d_1-1,k_0,k)$ linear independent domain, then for any $G_0\in \Ec_{k_0}(\Theta)$, it holds:
\begin{equation}
\liminf_{ \substack{G,H\overset{W_1}{\to} G_0\\ G\neq H\in \Gc_k(\Theta) }} \frac{\|G-H\|_{\Phi}}{\mbf_{2d_1-1}(G-\theta_0,H-\theta_0)} >0, \label{eqn:localinverseboundmoment}
\end{equation}
where $\theta_0$ is a arbitrary element in $\Rb^q$.
\item \label{itemb:thm:inverseboundmoment}
If $\myF$ is a $(2k-1,1,k)$ linear independent domain, then \eqref{eqn:localinverseboundmoment} holds for any $G_0\in \Gc_{k_0}(\Theta)$ for any $k_0\in [k]$. %\myred{to be typed: optimality of $2d_1-1$ in the denominator} requires the orders of limit and sup is exchangeable
\item \label{itemc:thm:inverseboundmoment}
Suppose 
$$
\sup_{|\alpha|\leq 2d_1-1} \sup_{\theta\in \Theta} \sup_{\myf\in\myF} \left| D^\alpha \myf(\theta) \right|<\infty
$$
and that
there is a uniform continuity modulus $w(\cdot)$ such that: for any $\alpha$ with $|\alpha|=m$,  
$$\sup_{\myf\in \myF}|D^\alpha \myf(\theta) - D^\alpha \myf(\theta')|\leq w(\theta-\theta')$$ 
with $\lim_{h\to 0}  w(h) =0$. Then
\begin{equation}
\limsup_{ \substack{G,H\overset{W_1}{\to} G_0\\ G\neq H\in \Gc_k(\Theta) }} \frac{\|G-H\|_{\Phi}}{\mbf_{2d_1-1}(G-\theta_0,H-\theta_0)} <\infty. 
\label{eqn:localinverseboundmomentupp}
\end{equation}
where $\theta_0$ is a arbitrary element in $\Rb^q$. 
%\color{blue}{LN: again for arbitrary element $\theta_0 \in \Rb^q$ YW: done}
\end{enumerate}
\end{thm}

The above theorem basically states that  $\|G-H\|_{\Phi}$, the distance between mixture densities, which will be discussed in detailed in Section \ref{sec:MMD1}, is roughly the same as $\mbf_{2d_1-1}(G-\theta_0,H-\theta_0)$, the moment difference between the corresponding mixing measures. Specifically, given some regularity condition specified in parts \ref{itema:thm:inverseboundmoment} and \ref{itemc:thm:inverseboundmoment}, it then holds that in a small neighborhood around $G_0$: for some constant $c,C$,
\begin{align*}
\numberthis \label{eqn:locinfgeo}
c\mbf_{2d_1-1}(G-\theta_0,H-\theta_0)  \leq & \|G-H\|_{\Phi} \\
\leq & C \mbf_{2d_1-1}(G-\theta_0,H-\theta_0) 
\end{align*}
for any $G$ and $H$ in the neighborhood. Recall $d_1=2(k-k_0+1)-1$ depends on the number of component $k_0$ of $G_0$. If more differentiability conditions as in part \ref{itemb:thm:inverseboundmoment} and $\Gc_k(\Theta)$ is distinguishable by $\myF$, then it also holds that 
\begin{align*}
\numberthis \label{eqn:glabalequimoment}
c\mbf_{2k-1}(G-\theta_0,H-\theta_0)  \leq & \|G-H\|_{\Phi} \\
\leq & C \mbf_{2k-1}(G-\theta_0,H-\theta_0)  
\end{align*}
for any $G,H\in \Gc_k(\Theta)$. 


\begin{rem}
The inequalities in Eq.\eqref{eqn:glabalequimoment} (Eq. \eqref{eqn:locinfgeo}) demonstrate that the moment difference of mixing measures is an intrinsic metric that captures precisely the global (local) geometry of data population densities, under a (relaxed) condition of strongly identifiable finite mixtures,  %\textcolor{blue}{YW: how about change to "the regularity condition specified in the theorems", since one of the contribution of our paper is to weaken the standard strong identifiability condition}, 
even though the
Wasserstein distance arguably continues to be an appealing surrogate for measuring the quality of the model's parameter estimates. 
In fact, by Lemma \ref{lem:momentbound} we know that the moment difference is an upper bound for Wasserstein distance between mixing measures, and consequently, upper bounds for estimation errors in terms of moment difference will automatically yield the same upper bounds for estimation errors in terms of Wasserstein distance. Moreover, since Theorem \ref{thm:inverseboundmoment} provides an inverse bound in terms of the moment difference, as we have done in Theorem \ref{thm:convergencerate} we can restate all the remaining examples in this section %Section \ref{sec:examples} 
in terms of estimation errors defined via moment difference, which are strictly speaking stronger results as discussed in the previous sentence. 
\myeoe
%However, due to the prevalence of the vast existing literature on using Wasserstein distance to measure estimation errors of mixing measures, we still present these results in terms of Wasserstein distance, and just make a remark here that all of them can be replaced with moment difference. 
\end{rem}

\begin{rem}
\label{rem:infgeocom}
    There is some related work on quantifying the distances between mixing measures. For location Gaussian mixtures, \cite[Theorem 4.2]{doss2020optimal} establishes a similar inequality \textcolor{blue}{to \eqref{eqn:glabalequimoment}} for squared Hellinger distance, KL divergence, and $\chi^2$-divergence. It is noteworthy that their results, by leveraging special properties of the Gaussian distribution, quantify how the constant coefficients depend on $q$ and $k$. However, it is not straightforward to see how their proof can be generalized beyond location Gaussian mixtures. Another related work is \cite{gassiat2014local} where they quantify the local geometry with respect to Hellinger distance of general location mixtures by a pseudo metric. 
The strength of Theorem \ref{thm:inverseboundmoment} is that it is applicable to general mixture models and a general integral probability metric, which extend beyond either location Gaussian mixtures or location mixtures considered in such prior work. For instance, one can easily obtain sufficient conditions for general mixture models to obtain Eq.\eqref{eqn:glabalequimoment} (Eq. \eqref{eqn:locinfgeo}) type inequality with $\|G-H\|_{\Phi}$ specialized to KS distance (see \cite[Section~3.1.1]{wei2023minimum}), MMD (see Section \ref{sec:MMD1}), total variational distance (see \cite[Section~7.1]{wei2023minimum}), and beyond; we leave the details to interested readers. Furthermore, the local type inequality \eqref{eqn:locinfgeo} appears to be novel, to the best of our knowledge. %\marginpar{blue one is newly added} 
\myeoe
\end{rem}
